Deriving Correct High-Performance Algorithms

Dijkstra observed that verifying correctness of a program is difficult and conjectured that derivation of a program hand-in-hand with its proof of correctness was the answer. We illustrate this goal-oriented approach by applying it to the domain of dense linear algebra libraries for distributed memory parallel computers. We show that algorithms that underlie the implementation of most functionality for this domain can be systematically derived to be correct. The benefit is that an entire family of algorithms for an operation is discovered so that the best algorithm for a given architecture can be chosen. This approach is very practical: Ideas inspired by it have been used to rewrite the dense linear algebra software stack starting below the Basic Linear Algebra Subprograms (BLAS) and reaching up through the Elemental distributed memory library, and every level in between. The paper demonstrates how formal methods and rigorous mathematical techniques for correctness impact HPC.

==> GenEigTransform.tex <==
\resetsteps      % Reset all the commands to create a blank worksheet  

% Define the operation to be computed

\renewcommand{\routinename}{ A := L^{-1} A L^{-H} }

% Step 3: Loop-guard 

\renewcommand{\guard}{
  m( A_{TL} ) < m( A )
}

% Step 4: Define Initialize 

\renewcommand{\partitionings}{
  $
  A \rightarrow
  \FlaTwoByTwo{A_{TL}}{A_{TR}}
              {A_{BL}}{A_{BR}}
  $
,
  $
  L \rightarrow
  \FlaTwoByTwo{L_{TL}}{L_{TR}}
              {L_{BL}}{L_{BR}}
  $
,
  $
  Y \rightarrow
  \FlaTwoByTwo{Y_{TL}}{Y_{TR}}
              {Y_{BL}}{Y_{BR}}
  $
}

\renewcommand{\partitionsizes}{
$ A_{TL} $,
$ L_{TL} $, and $ Y_{TL} $ are $ 0 \times 0 $.  Initially, $ Y = 0 $.
}

% Step 5a: Repartition the operands 

\renewcommand{\blocksize}{b}

\renewcommand{\repartitionings}{
$
  \FlaTwoByTwo{A_{TL}}{ \star }
              {A_{BL}}{A_{BR}}
  \rightarrow
  \FlaThreeByThreeBR{A_{00}}{ \star }{ \star }
                    {A_{10}}{A_{11}}{ \star }
                    {A_{20}}{A_{21}}{A_{22}}
$,
$
  \FlaTwoByTwo{L_{TL}}{ 0 }
              {L_{BL}}{L_{BR}}
  \rightarrow
  \FlaThreeByThreeBR{L_{00}}{0}{0}
                    {L_{10}}{L_{11}}{0}
                    {L_{20}}{L_{21}}{L_{22}}
$, \\
$
  \FlaTwoByTwo{Y_{TL}}{ 0 }
              {Y_{BL}}{Y_{BR}}
  \rightarrow
  \FlaThreeByThreeBR{Y_{00}}{0}{0}
                    {Y_{10}}{Y_{11}}{0}
                    {Y_{20}}{Y_{21}}{Y_{22}}
$
}

\renewcommand{\repartitionsizes}{
  $ A_{11} $,
  $ L_{11} $, and $ Y_{11} $ are $ b \times b $
}

% Step 5b: Move the double lines 

\renewcommand{\moveboundaries}{
$
  \FlaTwoByTwo{A_{TL}}{ \star }
              {A_{BL}}{A_{BR}}
  \leftarrow
  \FlaThreeByThreeTL{A_{00}}{ \star }{ \star }
                    {A_{10}}{A_{11}}{ \star }
                    {A_{20}}{A_{21}}{A_{22}}
$,
$
  \FlaTwoByTwo{L_{TL}}{0}
              {L_{BL}}{L_{BR}}
  \leftarrow
  \FlaThreeByThreeTL{L_{00}}{0}{0}
                    {L_{10}}{L_{11}}{0}
                    {L_{20}}{L_{21}}{L_{22}}
$, \\
$
  \FlaTwoByTwo{Y_{TL}}{0}
              {Y_{BL}}{Y_{BR}}
  \leftarrow
  \FlaThreeByThreeTL{Y_{00}}{0}{0}
                    {Y_{10}}{Y_{11}}{0}
                    {Y_{20}}{Y_{21}}{Y_{22}}
$}

% Step 8: Insert the updates required to change the 
%         state from that given in Step 6 to that given in Step 7
% Note: The below needs editing!!!

\renewcommand{\update}{
\begin{tabular}{| l @{}| l @{}|} \hline
\underline{Variant 1} &
\underline{Variant 2} \\
$  \begin{array}[t]{l}
\rowcolor[gray]{0.8}    Y_{10} \becomes L_{10} A_{00} ~~~ \mbox{({\sc hemm})} \\
\rowcolor[gray]{0.8}    A_{10} \becomes A_{10} L_{00}^{-H} ~~~ \mbox{({\sc trsm})} \\
    A_{10} \becomes W_{10} = A_{10} - \frac{1}{2} Y_{10} \\
    A_{11} \becomes A_{11} - ( A_{10} L_{10}^H + L_{10} A_{10}^H) \\
    A_{11} \becomes L_{11}^{-1} A_{11} L_{11}^{-H}\\
    A_{10} \becomes A_{10} - \frac{1}{2} Y_{10}\\
    A_{10} \becomes L_{11}^{-1} A_{10}
  \end{array}
$
&
$
  \begin{array}[t]{l}
\rowcolor[gray]{0.8}    Y_{10} \becomes L_{10} A_{00} ~~~ \mbox{({\sc hemm})} \\
    A_{10} \becomes W_{10} = A_{10} - \frac{1}{2} Y_{10} \\
    A_{11} \becomes A_{11} - ( A_{10} L_{10}^H + L_{10} A_{10}^H )  \\
    A_{11} \becomes L_{11}^{-1}  A_{11} L_{11}^{-H} \\
\rowcolor[gray]{0.8}    A_{21} \becomes A_{21} - A_{20} L_{10}^H ~~~ \mbox{({\sc gemm})} \\
    A_{21} \becomes A_{21} L_{11}^{-H} \\
    A_{10} \becomes A_{10} - \frac{1}{2}  Y_{10} \\
    A_{10} \becomes L_{11}^{-1} A_{10} \\
  \end{array}
$
\\ \hline
\underline{Variant 3}
&
\underline{Variant 4} \\
$
  \begin{array}[t]{l}
    A_{10} \becomes W_{10} = A_{10} - \frac{1}{2} Y_{10} \\
    A_{11} = A_{11} - ( A_{10} L_{10}^H + L_{10} A_{10}^H ) \\
    A_{11} = L_{11}^{-1} A_{11} L_{11}^{-H}\\
\rowcolor[gray]{0.8}    A_{21} = A_{21} - A_{20} L_{10}^H ~~~ \mbox{({\sc gemm})} \\
    A_{21} = A_{21} L_{11}^{-H} \\
    A_{10} = A_{10} - \frac{1}{2} Y_{10} \\
    A_{10} = L_{11}^{-1} A_{10}\\
\rowcolor[gray]{0.8}        Y_{20} = Y_{20} + L_{21} A_{10} ~~~ \mbox{({\sc gemm})}    \\
    Y_{21} = L_{21} A_{11}\\
\rowcolor[gray]{0.8}    Y_{21} = Y_{21} + L_{20} A_{10}^H ~~~ \mbox{({\sc gemm})}
\end{array}
$
&
$
  \begin{array}[t]{l}
%
%    A10 = L11 \ A10;
%
    A_{10} \becomes L_{11}^{-1} A_{10} \\
%
%    A20 = A20 - L21 * A10;
%
\rowcolor[gray]{0.8}    A_{20} \becomes A_{20} - L_{21} A_{10} ~~~ \mbox{({\sc gemm})} \\
%
%    A11 = L11 \ A11 / L11';
%
    A_{11} \becomes L_{11}^{-1} A_{11} L_{11}^{-H} \\
%
%    Y21 = - 0.5 *  L21 * A11;
%
    Y_{21} \becomes L_{21} A_{11} \\
%
%    A21 = A21 / L11' + Y21;
%    W21 = A21;
%
    A_{21} \becomes A_{21} L_{11}^{-H} \\
    A_{21} \becomes W_{21} = A_{21} - \frac{1}{2} Y_{21} \\
%
%    A22 = A22 - ( L21 * W21' + W21 * L21' );
%
\rowcolor[gray]{0.8}    A_{22} \becomes A_{22} - ( L_{21} A_{21}^H + A_{21} L_{21}^H ) ~~~ \mbox{({\sc her2k})} \\
%    A21 =  A21 + Y21;
    A_{21} \becomes A_{21} - \frac{1}{2} Y_{21}  \\
  \end{array}
$ \\ \hline
\multicolumn{2}{|l|}{
\underline{Variant 5}} \\
\multicolumn{2}{|l|}
{$
  \begin{array}[t]{l}
    A_{11} \becomes L_{11}^{-1} A_{11} L_{11}^{-H} \\
    Y_{21} \becomes L_{21} A_{11} \\
    A_{21} \becomes A_{21} L_{11}^{-H} \\
    A_{21} \becomes W_{21} = A_{21} - \frac{1}{2} Y_{21} \\
\rowcolor[gray]{0.8}    A_{22} \becomes A_{22} - ( L_{21} A_{21}^H + A_{21} L_{21}^H ) ~~~ \mbox{({\sc her2k})} \\
    A_{21} \becomes A_{21} - \frac{1}{2} Y_{21}  \\
\rowcolor[gray]{0.8}    A_{21} \becomes L_{22}^{-1} A_{21} ~~~ \mbox{({\sc trsm})}
  \end{array}
$} \\ \hline
\end{tabular}}

\begin{figure}[tbp]

\FlaAlgorithmNarrow

\caption{Blocked algorithms for computing $ A \becomes L^{-1} A L^{-H} $.}
\label{fig:algs}
\end{figure}


==> GenEigTransform2.tex <==
\resetsteps      % Reset all the commands to create a blank worksheet  

% Define the operation to be computed

\renewcommand{\routinename}{ A := L^H A L }

% Step 3: Loop-guard 

\renewcommand{\guard}{
  m( A_{TL} ) < m( A )
}

% Step 4: Define Initialize 

\renewcommand{\partitionings}{
  $
  A \rightarrow
  \FlaTwoByTwo{A_{TL}}{A_{TR}}
              {A_{BL}}{A_{BR}}
  $
,
  $
  L \rightarrow
  \FlaTwoByTwo{L_{TL}}{L_{TR}}
              {L_{BL}}{L_{BR}}
  $
}

\renewcommand{\partitionsizes}{
$ A_{TL} $ and
$ L_{TL} $ are $ 0 \times 0 $.
}

% Step 5a: Repartition the operands 

\renewcommand{\blocksize}{b}

\renewcommand{\repartitionings}{
$
  \FlaTwoByTwo{A_{TL}}{ \star }
              {A_{BL}}{A_{BR}}
  \rightarrow
  \FlaThreeByThreeBR{A_{00}}{ \star }{ \star }
                    {A_{10}}{A_{11}}{ \star }
                    {A_{20}}{A_{21}}{A_{22}}
$,
$
  \FlaTwoByTwo{L_{TL}}{ 0 }
              {L_{BL}}{L_{BR}}
  \rightarrow
  \FlaThreeByThreeBR{L_{00}}{0}{0}
                    {L_{10}}{L_{11}}{0}
                    {L_{20}}{L_{21}}{L_{22}}
$
}

\renewcommand{\repartitionsizes}{
  $ A_{11} $ and
  $ L_{11} $ are $ b \times b $
}

% Step 5b: Move the double lines 

\renewcommand{\moveboundaries}{
$
  \FlaTwoByTwo{A_{TL}}{ \star }
              {A_{BL}}{A_{BR}}
  \leftarrow
  \FlaThreeByThreeTL{A_{00}}{ \star }{ \star }
                    {A_{10}}{A_{11}}{ \star }
                    {A_{20}}{A_{21}}{A_{22}}
$,
$
  \FlaTwoByTwo{L_{TL}}{0}
              {L_{BL}}{L_{BR}}
  \leftarrow
  \FlaThreeByThreeTL{L_{00}}{0}{0}
                    {L_{10}}{L_{11}}{0}
                    {L_{20}}{L_{21}}{L_{22}}
$
}

% Step 8: Insert the updates required to change the 
%         state from that given in Step 6 to that given in Step 7
% Note: The below needs editing!!!

\renewcommand{\update}{
\begin{tabular}{| @{\hspace{2.75pt}} l @{}|@{\hspace{2.75pt}} l @{}|} \hline
\underline{Variant 1} &
\underline{Variant 2} \\
$  \begin{array}[t]{@{}l}
    Y_{10} \becomes A_{11} L_{10} \\
\rowcolor[gray]{0.8}    A_{10} \becomes A_{10} L_{00} ~~~ \mbox{({\sc trmm})}\\
    A_{10} \becomes W_{10} = A_{10} + \frac{1}{2} Y_{10}\\
\rowcolor[gray]{0.8}    A_{00} \becomes A_{00} + ( A_{10}^H L_{10} + L_{10}^H A_{10} ) ~~~ \mbox{({\sc her2k})} \\
    A_{10} \becomes A_{10} + \frac{1}{2} Y_{10} \\
    A_{10} \becomes L_{11}^H  A_{10} \\
    A_{11} \becomes L_{11}^H A_{11} L_{11}\\
  \end{array}
$
&
$
  \begin{array}[t]{@{}l}
    Y_{10} \becomes A_{11} L_{10} \\
    A_{10} \becomes W_{10} = A_{10} + \frac{1}{2} Y_{10}\\
\rowcolor[gray]{0.8}    A_{00} \becomes A_{00} + ( A_{10}^H L_{10} + L_{10}^H A_{10} ) ~~~ \mbox{({\sc her2k})} \\
    A_{10} \becomes A_{10} + \frac{1}{2} Y_{10} \\
    A_{10} \becomes L_{11}^H  A_{10} \\
    A_{11} \becomes L_{11}^H A_{11} L_{11}\\
\rowcolor[gray]{0.8}    A_{20} \becomes A_{20} + A_{21} L_{10} ~~~ \mbox{({\sc gemm})} \\
    A_{21} \becomes A_{21} L_{11}\\
  \end{array}
$
\\ \hline
\underline{Variant 3} 
&
\underline{Variant 4 (new)} 
\\
$
  \begin{array}[t]{@{}l}
\rowcolor[gray]{0.8}    Y_{21} \becomes A_{22} L_{21} ~~~ \mbox{({\sc hemm})} \\
    A_{21} \becomes A_{21} L_{11} \\
    A_{21} \becomes W_{21} = A_{21} + \frac{1}{2} Y_{21}\\
    A_{11} \becomes L_{11}^H A_{11} L_{11}\\
    A_{11} \becomes A_{11} + ( A_{21}^H L_{21} + L_{21}^H A_{21} )\\
    A_{21} \becomes A_{21} + \frac{1}{2} Y_{21}\\
\rowcolor[gray]{0.8}    A_{21} \becomes L_{22}^H A_{21} ~~~ \mbox{({\sc trmm})}
\end{array}
$
&
$
  \begin{array}[t]{@{}l}
    A_{10} = L_{11}^H A_{10} \\
\rowcolor[gray]{0.8}    A_{10} = A_{10} + L_{21}^H * A_{20} ~~~ \mbox{({\sc gemm})} \\
\rowcolor[gray]{0.8}    Y_{21} = A_{22} L_{21}~~~ \mbox{({\sc hemm})} \\
    A_{21} = A_{21} L_{11} \\
    A_{21} = A_{21} + 0.5 * Y_{21} \\
    A_{11} = L_{11}^H A_{11} L_{11} \\
    A_{11} = A_{11} + ( A_{21}^H L_{21} + L_{21}^H * A_{21} \\
    A_{21} = A_{21} + 0.5 * Y_{21}
\end{array}
$
\\ \hline
\end{tabular}}

\begin{figure}[tbp]

\FlaAlgorithmNarrow

\caption{Blocked algorithms for computing $ A \becomes L^H A L $.}
\label{fig:algs2}
\end{figure}


==> GenEigTransformBoth.tex <==
\begin{figure*}[tbp]

\begin{tabular}{| l @{} | l @{} | l @{}|} \hline
\underline{Variant 1} 
&
\underline{Variant 2}
& 
\underline{Variant 3}
\\
$  \begin{array}[t]{l}
\rowcolor[gray]{0.8}    Y_{10} \becomes L_{10} A_{00} ~~~ \mbox{({\sc hemm})} \\
\rowcolor[gray]{0.8}    A_{10} \becomes A_{10} L_{00}^{-H} ~~~ \mbox{({\sc trsm})} \\
    A_{10} \becomes W_{10} = A_{10} - \frac{1}{2} Y_{10} \\
    A_{11} \becomes A_{11} - ( A_{10} L_{10}^H + L_{10} A_{10}^H) \\
    A_{11} \becomes L_{11}^{-1} A_{11} L_{11}^{-H}\\
    A_{10} \becomes A_{10} - \frac{1}{2} Y_{10}\\
    A_{10} \becomes L_{11}^{-1} A_{10}
  \end{array}
$ 
&
$
  \begin{array}[t]{l}
\rowcolor[gray]{0.8}    Y_{10} \becomes L_{10} A_{00} ~~~ \mbox{({\sc hemm})} \\
    A_{10} \becomes W_{10} = A_{10} - \frac{1}{2} Y_{10} \\
    A_{11} \becomes A_{11} - ( A_{10} L_{10}^H + L_{10} A_{10}^H )  \\
    A_{11} \becomes L_{11}^{-1}  A_{11} L_{11}^{-H} \\
\rowcolor[gray]{0.8}    A_{21} \becomes A_{21} - A_{20} L_{10}^H ~~~ \mbox{({\sc gemm})} \\
    A_{21} \becomes A_{21} L_{11}^{-H} \\
    A_{10} \becomes A_{10} - \frac{1}{2}  Y_{10} \\
    A_{10} \becomes L_{11}^{-1} A_{10} \\
  \end{array}
$
&
$
  \begin{array}[t]{l}
    A_{10} \becomes W_{10} = A_{10} - \frac{1}{2} Y_{10} \\
    A_{11} = A_{11} - ( A_{10} L_{10}^H + L_{10} A_{10}^H ) \\
    A_{11} = L_{11}^{-1} A_{11} L_{11}^{-H}\\
\rowcolor[gray]{0.8}    A_{21} = A_{21} - A_{20} L_{10}^H ~~~ \mbox{({\sc gemm})} \\
    A_{21} = A_{21} L_{11}^{-H} \\
    A_{10} = A_{10} - \frac{1}{2} Y_{10} \\
    A_{10} = L_{11}^{-1} A_{10}\\
\rowcolor[gray]{0.8}        Y_{20} = Y_{20} + L_{21} A_{10} ~~~ \mbox{({\sc gemm})}    \\
    Y_{21} = L_{21} A_{11}\\
\rowcolor[gray]{0.8}    Y_{21} = Y_{21} + L_{20} A_{10}^H ~~~ \mbox{({\sc gemm})}
\end{array}
$
\\ \hline
\underline{Variant 4} 
&
\underline{Variant 5}
& 
\\
$
  \begin{array}[t]{l}
%
%    A10 = L11 \ A10;
%
    A_{10} \becomes L_{11}^{-1} A_{10} \\
%
%    A20 = A20 - L21 * A10;
%
\rowcolor[gray]{0.8}    A_{20} \becomes A_{20} - L_{21} A_{10} ~~~ \mbox{({\sc gemm})} \\
%
%    A11 = L11 \ A11 / L11';
%
    A_{11} \becomes L_{11}^{-1} A_{11} L_{11}^{-H} \\
%
%    Y21 = - 0.5 *  L21 * A11;
%
    Y_{21} \becomes L_{21} A_{11} \\
%
%    A21 = A21 / L11' + Y21;
%    W21 = A21;
%
    A_{21} \becomes A_{21} L_{11}^{-H} \\
    A_{21} \becomes W_{21} = A_{21} - \frac{1}{2} Y_{21} \\
%
%    A22 = A22 - ( L21 * W21' + W21 * L21' );
%
\rowcolor[gray]{0.8}    A_{22} \becomes A_{22} - ( L_{21} A_{21}^H + A_{21} L_{21}^H ) ~~~ \mbox{({\sc her2k})} \\
%    A21 =  A21 + Y21;
    A_{21} \becomes A_{21} - \frac{1}{2} Y_{21}  \\
  \end{array}
$
&
$
  \begin{array}[t]{l}
    A_{11} \becomes L_{11}^{-1} A_{11} L_{11}^{-H} \\
    Y_{21} \becomes L_{21} A_{11} \\
    A_{21} \becomes A_{21} L_{11}^{-H} \\
    A_{21} \becomes W_{21} = A_{21} - \frac{1}{2} Y_{21} \\
\rowcolor[gray]{0.8}    A_{22} \becomes A_{22} - ( L_{21} A_{21}^H + A_{21} L_{21}^H ) ~~~ \mbox{({\sc her2k})} \\
    A_{21} \becomes A_{21} - \frac{1}{2} Y_{21}  \\
\rowcolor[gray]{0.8}    A_{21} \becomes L_{22}^{-1} A_{21} ~~~ \mbox{({\sc trsm})}
  \end{array}
$
&
\\ \hline
\end{tabular}

\caption{All algorithms corresponding to the Invariants in Figures~\ref{fig:invariants} and~\ref{fig:invariants2} for both  $ A \becomes L^{-1} A L^{-H} $ and 
$ A \becomes L^H A L $.}
\label{fig:algsboth}
\end{figure*}


==> alg2.tex <==
In this section, we derive algorithms for computing $ C \becomes L^H A L $, overwriting the lower triangular part of Hermitian matrix $ A $.

\vspace{0.05in}
\noindent
{\bf Derivation.}
%\subsection{Derivation}
We once again give the minimum information required so that those
familiar with the FLAME methodology understand how the algorithms
were derived.  
%Subsection~\ref{sec:discussion2}.

\input invariants2
% \input GenEigTransform2

The postcondition for this operation is given
by  $ A = L^H \hat A L $ 
where, again, $ \hat{A} $ represents the input matrix
$ A $.  
We partition the matrices so that
\[
A \rightarrow
\FlaTwoByTwo 
 { A_{TL} }{ \star }
 { A_{BL} }{ A_{BR} },
\quad
\mbox{and}
\quad
L \rightarrow
\FlaTwoByTwo 
 { L_{TL} }{ 0 }
 { L_{BL} }{ L_{BR} },
\]
where $ A_{TL} $ and $ L_{TL} $ are square submatrices and
$ \star $ denotes the parts of the Hermitian matrices that are neither stored nor updated.
Substituting these partitioned matrices into the postcondition yields the PME
\begin{eqnarray*}
%%% \lefteqn{
\FlaTwoByTwo 
 { A_{TL} }{ \star }
 { A_{BL} }{ A_{BR} }
%%% = 
%%% \FlaTwoByTwo 
%%%  { \begin{array}[t]{r}
%%%    L_{TL} \hat A_{TL} L_{TL}^H + L_{BL}^H \hat A_{BL} L_{TL} +  \\
%%%    L_{TL}^H \hat A_{BL}^H L_{BL} + L_{BL}^H \hat A_{BR} L_{BL} 
%%% \  \end{array}}
%%%  { \star } 
%%%  { L_{BR}^H ( \hat A_{BL} L_{TL} + \hat A_{BR} L_{BL} ) } 
%%%  { L_{BR}^H \hat A_{BR} L_{BR} } } \hspace{0.75in} \\
%%% & &
=  
\FlaTwoByTwo 
 { L_{TL}^H \hat A_{TL} L_{TL} + ( W_{BL}^H L_{BL} + L_{BL}^H W_{BL} ) }{ \star }
 { L_{BR}^H ( \hat A_{BL} L_{TL} + \hat A_{BR} L_{BL} ) } 
 { L_{BR}^H \hat A_{BR} L_{BR} } 
,
\end{eqnarray*}
where
$ W_{BL} = 
\hat A_{BL} L_{TL} + \frac{1}{2} \hat A_{BR} L_{BL} $.
Letting $ Y_{BL} = \hat A_{BR} L_{BL} $ yields five loop invariants
for this operation
that exploit and maintain symmetry.
These loop invariants are listed in Figure~\ref{fig:invariants2}
while the corresponding blocked algorithms were already given in
Figures~\ref{fig:algs} and~\ref{fig:algsboth}.
One of the loop invariants yields
an algorithm that incurs $ O( n^3) $ additional computation and
we do not give the related algorithm.


\vspace{0.05in}
\noindent
{\bf Discussion.}
%\subsection{Discussion}
%\label{sec:discussion2}
For this operation, in principle, all of the highlighted suboperations
can be implemented to be scalable on parallel architectures.

% \input GenEigTransformBoth


==> conclusion_final.tex <==
We have systematically derived and presented a multitude of algorithms for the 
transformation of the generalized Hermitian-definite eigenvalue problem to the 
standard Hermitian eigenvalue problem. While the concept of avoiding the 
unscalability in the traditional algorithm for $A := L^{-1} A L^H$ was 
already discussed in the paper by Sears et al., we give a clear
%derivation of such that algorithm as well as several other new algorithmic 
derivation of that algorithm as well as several other new algorithmic 
possibilities.
For $ A \becomes L^H A L $ we similarly present several algorithms, including
one that is different from that used by ScaLAPACK and achieves superior performance.

The performance improvements of Elemental over ScaLAPACK are not the
central message of this paper.
%It is that the combination of a systematic 
%method for deriving algorithms and a highly programmable library has
%allowed us to thoroughly explore the performance of a wide variety of 
%approaches.
Instead, we argue that a systematic method for deriving algorithms combined
with a highly-programmable library has allowed us to thoroughly explore the
performance of a wide variety of algorithms.
Still, Elemental outperforms ScaLAPACK even when
the same algorithm is used and hence Elemental is clearly faster 
on this architecture.
%% almost a necessary 
%our exhaustive approach.
%a consequence of this.
% 

\subsection*{Availability}
The Elemental library
can be found at
\begin{center}
{\tt http://code.google.com/p/elemental}.
\end{center}
This library includes all discussed variants for single, double,
complex, and double complex datatypes, and for updating either the
upper or lower triangular parts of $ A $.  The algorithms are also
implemented as part of the {\tt libflame} library~\cite{libflame_ref} (a modern
replacement library for LAPACK) including
algorithm-by-blocks that can be scheduled for parallel execution on
multi-threaded and/or multi-GPU accelerated architectures via the
SuperMatrix runtime system~\cite{Quintana:2008:PMA,FLAWN50,SuperMatrix:PPoPP09}.
M-script implementations for Matlab and Octave can be found at
\begin{center}
{\tt http://www.cs.utexas.edu/users/flame/Extras/FLAWN56/}.
\end{center}



==> intro.tex <==
The generalized Hermitian-definite eigenvalue problem occurs in one of three forms:
$Ax=\lambda Bx$, $ABx=\lambda x$, and $BAx=\lambda x$, where $A$ is Hermitian
and $B$ is Hermitian and positive-definite.  The usual solution strategy for
each of these problems is to exploit the positive-definiteness of $B$ in order
to compute its Cholesky factorization and transform the problem into a 
standard Hermitian eigenvalue problem, solve the Hermitian eigenproblem, 
and then backtransform the eigenvectors if necessary.

In particular, the following steps are performed for the $A x = \lambda B x$
case:
%%% \begin{itemize}
%%% \item
(1)
Compute the Cholesky factorization $ B = L L^H $.
%%% This step requires approximately $ \frac{1}{3} n^3 $ floating point operations%
%%% \footnote{Here we count a floating point  multiply or add of any type (single, double, complex) as one floating point operation (flops).  In practice, a double precision complex multiply or add requires four double precision real floating point operations, making the cost for complex arithmetic four times as expensive.
%%% More on this in Section~\ref{sec:performance}.}.%
%%% \item
%%% \label{step:Trans}
(2) Transform $ C \becomes L^{-1} A L^{-H} $ so that $ A x = \lambda B x $ is
transformed to $ C y = \lambda y $ with $ y = L^{-H} x $.
%%% Cost: approximately $ n^3 $ flops.
%%% \item
%%% \label{step:TriRed}
(3) Reduce $ C $ to tridiagonal form: $ C \becomes Q_C T Q_C^H $ where $ Q_C $ is unitary
and $ T $ is tridiagonal.
%%% Cost: approximately $ \frac{4}{3} n^3 $ flops.
%%% \item
%%% \label{step:TriEig}
(4) Compute the spectral decomposition of $ T $: $ T \becomes Q_T D Q_T^H $ where $ Q_T $ is unitary and $ D $ is diagonal.
%%% Cost: $ O( n^2 ) $ flops.
%%% \item
(5) Form $ X \becomes L Q_C Q_T $ so that
$
A X = B X D
$.
%%%  at a cost of about $ \frac{13}{3} n^3 $ flops
%%% ($ \frac{4}{3} n^3 $ to form $ Q_C $, $ 2 n^3 $ to form $ Q_C Q_T $ and
%%% $ n^3 $ to compute $ L ( Q_C Q_T ) $.).  {\bf This is not correct.  One should apply the Householder transforms that comprise $ Q_C $ to $ Q_T $ and then form $ L ( Q_C Q_T ) $.}
%%% \end{enumerate}
Then the eigenvalues can be found on the diagonal of $ D $ and the 
corresponding eigenvectors as the columns of $ X $.
In this paper, we focus on Step~2.  For the other two forms of the generalized Hermitian-definite eigenvalue problem this step becomes $ C \becomes L^H A L $.  Typically $ C $ overwrites matrix $ A $.
The present paper 
demonstrates how Elemental benefits from 
the FLAME methodology~\cite{FLAME_WoCo,Gunnels:2001:FFL,Quintana-Orti:2003:FDA,TSoPMC,Bientinesi:2008:FAR}
by allowing families of algorithms for dense matrix computations
to be systematically derived and presented in a clear, concise fashion.
This results in the most complete exposition to date of algorithms for 
computing $ L^{-1} A L^{-H} $ and $ L^H A L $.

While a family of algorithms and their parallelization
for these operations is the primary focus of this paper, 
we also consider this paper the second in a series of papers
related to the Elemental library for dense matrix computations
on distributed memory architectures.  
The first paper~\cite{Elemental:TOMS}
gave a broad overview of the vision behind the design of the Elemental library
%% Although not explicitly discussed in this paper, this then results
%%in similarly clear and concise code, as an interested reader will 
%% see by looking at the source code.
and performance comparisons 
between
ScaLAPACK~\cite{ScaLAPACK} and Elemental for
%a cross-section of operations.
a representative subset of operations.
Since the comparison is not the main focus of that paper, the reader 
is left wondering 
as to how much of the improvement in performance 
is due to algorithm choice rather than implementation.
This paper answers that question for the discussed operations.
It thus adds to the body of evidence that Elemental may be a worthy 
successor to ScaLAPACK.

This paper is organized as follows.
In Sections~\ref{sec:InvLAInvLH} and~\ref{sec:LHAL}
we derive algorithms for computing $ L^{-1} A L^{-H} $ and 
$ L^H A L $, respectively.
In Section~\ref{sec:performance} we present results from
performance experiments on a large cluster.
Related work is discussed in Section~\ref{sec:related}
and concluding remarks are given in the final section.




==> invariants2.tex <==
\begin{figure}[tbp]
\renewcommand*\arraystretch{1.4}
\begin{center}
\begin{tabular}{| l |} \hline
\underline{Loop Invariant 1}\\
{
\footnotesize
{\setlength{\arraycolsep}{2pt}
$
 \FlaTwoByTwo 
 { A_{TL} }{ \star }
 { A_{BL} }{ A_{BR} }
=
\FlaTwoByTwo 
 { L_{TL}^H \hat A_{TL} L_{TL} + ( W_{BL}^H L_{BL} + L_{BL}^H W_{BL} ) }
% { C_{TL} }
 { \star }
 { L_{BR}^H ( \hat{A}_{BL} L_{TL} + \hat{A}_{BR} L_{BL} ) }
% { C_{BL} }
{ \hat A_{BR} }
$
}
}
\\ \hline
\underline{Loop Invariant 2} \\
{
\footnotesize
{\setlength{\arraycolsep}{2pt}
$
 \FlaTwoByTwo 
 { A_{TL} }{ \star }
 { A_{BL} }{ A_{BR} }
=
\FlaTwoByTwo 
{ L_{TL}^H \hat A_{TL} L_{TL} + ( W_{BL}^H L_{BL} + L_{BL}^H W_{BL} ) }
% { C_{TL} }
 { \star }
 { \hat{A}_{BL} L_{TL} + \hat{A}_{BR} L_{BL} }
{ \hat A_{BR} }
$
}
}
\\ \hline
\underline{Loop Invariant 3} \\
{
\footnotesize
{\setlength{\arraycolsep}{2pt}
$
 \FlaTwoByTwo 
 { A_{TL} }{ \star }
 { A_{BL} }{ A_{BR} }
=
\FlaTwoByTwo 
 { L_{TL}^H \hat A_{TL} L_{TL} }
 { \star }
 { \hat{A}_{BL} L_{TL} }
{ \hat A_{BR} }
\wedge 
 \FlaTwoByTwo 
 { Y_{TL} }{ }
 { Y_{BL} }{ Y_{BR} }
= 
 \FlaTwoByTwo 
 {  }{ }
 { \hat{A}_{BR} L_{BL} }{ ~~~~~ }
$
}
}
\\ \hline
\underline{Loop Invariant 4}  
\\
\footnotesize
{\setlength{\arraycolsep}{2pt}
$
 \FlaTwoByTwo 
 { A_{TL} }{ \star }
 { A_{BL} }{ A_{BR} }
=
\FlaTwoByTwo 
 { L_{TL}^H \hat A_{TL} L_{TL} }
 { \star }
 { \hat{A}_{BL} L_{TL} }{ \hat A_{BR} }
$
}
\\ \hline
\underline{Loop Invariant 5}  
\\
\footnotesize
{\setlength{\arraycolsep}{2pt}
$
 \FlaTwoByTwo 
 { A_{TL} }{ \star }
 { A_{BL} }{ A_{BR} }
=
\FlaTwoByTwo 
 { L_{TL}^H \hat A_{TL} L_{TL} }
 { \star }
 { \hat{A}_{BL} }{ \hat A_{BR} }
$
}
\\ \hline
\end{tabular}
\end{center}
\caption{Five loop invariants for computing $ A \becomes L^H A L $.}
\label{fig:invariants2}
\end{figure}




==> performance.tex <==
%%\input perf_fig_sygst_all


We now show the 
performance attained by the different variants
on a large distributed memory parallel architecture.
We compare implementations
that are part of the 
Elemental library to the implementations
of this operation that are part of
%ScaLAPACK {\tt netlib} version 1.8.  
%the {\tt netlib} distribution of ScaLAPACK version 1.8.
%version 1.8 of the {\tt netlib} distribution of ScaLAPACK.
{\tt netlib} ScaLAPACK Version 1.8.
These results were taken from a technical report~\cite{} written in 2011, collected on an architecture that has since been retired.  However, the results illustrate our point and we would expect them to be qualitatively similar on current architectures.  

The performance experiments were carried out on Argonne National Laboratory's 
IBM Blue Gene/P architecture.  Details on this distributed parallel computer and the experiments are not of great importance to this discussion.  They can be found in~\cite{bibid}.


ScaLAPACK~\cite{shpcc92,SIAM92:ScaLAPACK,ScaLAPACK,ScaLAPACK:Guide} was developed in
the 1990s as a distributed memory dense matrix library coded in
Fortran-77 in the style of LAPACK.  Again the details of how ScaLAPACK parallelizes is not particularly pertinent.  Performance graphs for ScaLAPACK are merely given to demonstrate that the more complete implementations that are part of Elemental are competitive to what was the state-of-the-art.  Again, details can be found in~\cite{bibid}.

\NoShow{
\begin{figure}[tb!]
\begin{center}
\footnotesize
\begin{tabular}{l @{\hspace{1pt}}|@{\hspace{2pt}} l}
\underline{Variant 4 (Elemental)} & \underline{Variant 4 (ScaLAPACK)} \\
$
  \begin{array}[t]{l}
    A_{10} \becomes L_{11}^{-1} A_{10} \\
\rowcolor[gray]{0.7}    A_{20} \becomes A_{20} - L_{21} A_{10} ~~~ \mbox{(gemm)} \\
\rowcolor[gray]{0.9}    A_{11} \becomes L_{11}^{-1} A_{11} L_{11}^{-H} \\
\rowcolor[gray]{1.0}
    Y_{21} \becomes L_{21} A_{11} \\
    A_{21} \becomes A_{21} L_{11}^{-H} \\
    A_{21} \becomes W_{21} = A_{21}  - \frac{1}{2} Y_{21} \\
\rowcolor[gray]{0.7}    A_{22} \becomes A_{22} - ( L_{21} A_{21}^H + A_{21} L_{21}^H ) ~~~ \mbox{(her2k)} \\
\rowcolor[gray]{1.0}
%    A21 =  A21 + Y21;
    A_{21} \becomes A_{21} - \frac{1}{2} Y_{21}  \\
  \end{array}
$ 
&
$
  \begin{array}[t]{l}
    G_{21} \becomes L_{21} \\
    R_{21} \becomes A_{21} \\
    S_{10} \becomes A_{10} \\
    R_{11} \becomes \mbox{tril}(A_{11}) \\
    G_{21} \becomes -G_{21} L_{11}^{-1} \\
    R_{21} \becomes R_{21} + \frac{1}{2} G_{21} A_{11} \\
    \rowcolor[gray]{0.7}  A_{22} \becomes A_{22} + G_{21} R_{21}^H + R_{21} G_{21}^H  ~~~ \mbox{(her2k)} \\
    \rowcolor[gray]{0.7}  A_{20} \becomes A_{20} + G_{21} S_{10} ~~~ \mbox{(gemm)} \\
    \rowcolor[gray]{1.0}
    A_{21} \becomes A_{21} + G_{21} R_{11} \\
    A_{10} \becomes L_{11}^{-1} A_{10} \\
    \rowcolor[gray]{0.9} 
\left. 
\begin{array}{@{}l}
\rowcolor[gray]{0.9}    C_{11} \becomes \mbox{tril}(A_{11}) \\
\rowcolor[gray]{0.9}    \mbox{triu}(C_{11}) := \mbox{tril}(C_{11})^H \\
\rowcolor[gray]{0.9}     C_{11} \becomes L_{11}^{-1} C_{11} \\
\rowcolor[gray]{0.9}     C_{11} \becomes C_{11} L_{11}^{-1} \\
\rowcolor[gray]{0.9}     \mbox{tril}(A_{11}) := \mbox{tril}(C_{11}) 
\end{array} 
\hspace{-0.05in}
\right\} A_{11} \becomes L_{11}^{-1} A_{11} L_{11}^{-H} \\
\rowcolor[gray]{1.0} 
    A_{21} \becomes A_{21} L_{11}^{-H}
  \end{array}
$ 
\end{tabular}
\vspace{0.1in}
\end{center}
\caption{Operations performed by Variant 4 
in Elemental (left) and ScaLAPACK (right).}
\label{fig:ElementalVsSL}
\end{figure}
}

The ScaLAPACK routines {\tt p[sd]sygst} and {\tt p[cz]hegst} implement Variant 5 from Figure~\ref{fig:algs}.  In addition, 
a vastly more efficient algorithm 
(essentially Variant 4 from Figure~\ref{fig:algs}) is implemented as the routines
{\tt p[sd]syngst} and 
{\tt p[cz]hengst}. 
Routines {\tt p[sd]syngst} and  {\tt p[cz]hengst}
appears to have been derived from the work by 
Sears et al.
%%%The algorithm in the paper by Sears et al.\ computes $ L^{-H} A L^{-1} $ 
%%%after having computed a somewhat unusual version of the Cholesky factorization:
%%% $ B = L^H L $.  The paper gives few clues about what motivated the 
%%% discovery of the algorithm.  The algorithm itself is presented as a 
%%% double-nested loop around vector operations so that even level-2 BLAS operations
%%% are not obvious. No blocked algorithm is given in the paper.  It is merely 
%%% mentioned that the unblocked algorithm that is given motivated a blocked 
%%%version.  The one hint at how the algorithm came to be is the mentioning of 
%%% ``Gauss transforms''. We conclude that the authors used the following insight:
%%% When factoring a square matrix $ A $ into its $ LU $ factorization, $ A = L U $,
%%% one can view the process as
%%% \[
%%% \begin{array}[t]{c}
%%% \underbrace{\hat{L}_{n-1} \cdots \hat{L}_0} \\
%%% L^{-1}
%%% \end{array}
%%% A = U ,
%%% \mbox{ where }
%%% \hat{L}_k
%%% = 
%%% \FlaThreeByThreeBR
%%%   { I_{k \times k} }{ 0 }{ 0 }
%%%   { 0 }{ 1 }{ 0 }
%%%   { 0 }{-l_{21}^{(k)}}{ I }
%%% \]
%%% is a Gauss transform.  (Here $ I_{k \times k} $ denotes a $ k \times k $
%%% identity matrix.)
%%% There is a simple relation between $ L $ and these Gauss transforms in that
%%% each $ l_{21}^{(k)} $ equals the corresponding subdiagonal elements of
%%% matrix $ L $.
%%% Thus, the inverse of a {\em unit} lower triangular matrix $ L $ can 
%%% be viewed as a sequence of Gauss transforms that are easily identified from
%%% the matrix $ L $.
%%% If one wishes to compute $ L^{-1} A L^{-H} $ one
%%% can instead compute
%%% $
%%% \left( \hat{L}_{n-1} \cdots \left( \hat{L}_0  A 
%%% \hat{L}_{0}^H \right) \cdots \hat{L}_{n-1}^H \right) $.
%%% %There are a few details beyond this insight, like how to modify this for the
%%% %$ L $ from the Cholesky factorization which is not unit lower triangular and
%%% %how to generalize this to a blocked algorithm.
%%% The paper contains a few details beyond this insight, like how to modify
%%% this algorithm for the $ L $ from the Cholesky factorization, which is not
%%% unit lower triangular, and how to generalize this to a blocked algorithm.
%%% %These are only barely discussed in~\cite{Sears98} nor will we discuss this here, since 
%%% %we have an alternative way for deriving the algorithm.
%%% However, these topics are only barely discussed in~\cite{Sears98}, and we
%%% choose to omit discussion here since we have an alternative way of deriving
%%% the algorithm.
%%% Hopefully, this gives the reader some idea of how the authors
%%% of~\cite{Sears98} may have derived
%%% their algorithm as an alternative to our derivation based on the
%%% FLAME methodology.  
%%% It appears that the routines {\tt p[sd]syngst} and {\tt p[cz]hengst} in ScaLAPACK were 
%%% derived from the work by Sears et al.. 

We view Elemental~\cite{bibid} as a modern replacement for ScaLAPACK and PLAPACK~\cite{PLAPACK}.
It is coded in C{\tt \footnotesize ++} in a style that resembles the FLAME/C API~\cite{FLAME:API} used to 
implement the {\tt libflame} library~\cite{libflame_ref,CiSE09} (a modern replacement for LAPACK, coded 
in C). 
Elemental uses a two-dimensional elemental distribution that
can be most easily described as the same distribution used by ScaLAPACK
except that $ b_{\rm distr} = 1 $. The algorithmic block size is not
restricted by the distribution block size.  Elemental uses a more flexible
layering so that calls to global BLAS-like operations can be easily fused, which
means that communication overhead can be somewhat reduced by combining
communications from within separate calls to BLAS-like operations.
See~\cite{Elemental:TOMS} for details.

\vspace{0.05in}
\noindent
%\subsection{Tuning}
%% As mentioned above, all variants of Elemental and ScaLAPACK were tested on 
%% one midplane of a Blue Gene/P using a $32 \times 64$ process grid.
Details of how both packages were tuned can be found in~\cite{bibid}.  For our discussion here it suffices to say that we believe the comparisons to be fair.  However, both packages have evolved over the last half decade, and hence only qualitative comparisons between algorithmic variants are of importance, rather than the performance of one package relative to the other.

% \input perf_fig_sygst_rl
% \input perf_fig_sygst_ll

%\subsection{Results}
In Figure~\ref{fig:perf:sygst_all_top} 
we report performance of the different variants for the studied computations.
All experiments were performed with real double-precision 
(64-bit) data. 

As expected,
the variants that cast a significant part of the computation in terms
of a triangular solve with multiple right-hand sides ({\sc trsm})
attain significantly worse performance.  Variant 4 performs best,
since it casts most computation in terms of a symmetric (Hermitian) rank-2$k$ update
($ A_{22} - ( L_{21} A_{21}^H + A_{21} L_{21}^H ) $)  
and general rank-$k$ update, ($ A_{20} - L_{21} A_{10} $), which are well-known to parallelize more naturally.
Variants 2 and 3 underperform since symmetric (Hermitian) or matrix-panel multiplies 
(matrix multiply where the result matrix is narrow),
like $ L_{10} A_{00} $, $ A_{21} - A_{20} L_{10}^H $, and
$ Y_{21} + L_{20} A_{10}^H $,
require local contributions to be summed (reduced) across processes,
a collective communication that often requires significantly more time than
the simpler duplications needed for rank-$k$ updates.
Also, the local matrix-panel multiply that underlies these parallel
operations is often less optimized than the 
local rank-$k$ update that underlies the parallel implementations of
the symmetric (Hermitian) rank-2$k$ and general rank-$k$ updates. 


We believe that ScaLAPACK's Variant 4 is slower than Elemental's Variant 4 
for two reasons:
(1) ScaLAPACK's implementation is layered on top of the PBLAS and 
therefore redundantly communicates data,
and (2) At the time of these experiments, ScaLAPACK had a 
hard-coded block size for the local updates of their parallel symmetric
(Hermitian) rank-2$k$ update that is therefore not a parameter that is
easily tuned in that package (and we did not tune it for that reason).
%The point is that part of the better performance attained by parallel 
%implementations comes from the proper choice of algorithm, part comes
%from the implementation details, and part comes from how easily
%the implementation can be tuned.
Thus, part of the increased performance attained
by parallel implementations stems from the proper choice of algorithm,
part is the result of implementation details, and part comes from how
easily the implementation can be tuned.





==> program.tex <==
% program.sty, Version 3.3.11
% Version History:
% 3.3.1: Fix name clash with new AmsTeX (\@prime)
% 3.3.2: Minor spacing tweaks. Added \sfvariables for a different style.
% 3.3.3: Added \| to the definition of \dospecials, so that | will
%        still work in a verbatim environment.
% 3.3.4: Added \ifVBarOutsideProgram switch -- The command \normalbaroutside
%        makes | to act normally outside the program environment
% 3.3.5: Bugfix (\lt was defined as > in maths mode!)
% 3.3.6: Minor bugfix: added \do\@ to \dospecials (for AmsTeX)
% 3.3.7: Restore catcode of _ (due to clash with \includegraphics)
% 3.3.8: Save/restore \@currentlabel when \ifNumberPrograms is true
% 3.3.9: Added \bigcaps command (submitted by Matteo Corti <corti@inf.ethz.ch>)
% 3.3.10: Changed \www command to use normal text rather than typewriter
%         Changed \FOREACH \ATEACH to use \@typename
%         Added \boldsubm (uses \boldsymbol instead of text \bf)
% 3.3.11: Changed the default style to \sfvariables, old style is \bfvariables
% 3.3.12: Fixed the interaction with \index and \makeindex (which uses |)
%
%
% A LaTeX2e style file for typesetting algorithms.
% Copyright 1991, 2007 Martin Ward
% Martin.Ward@durham.ac.uk, martin@gkc.org.uk
% http://www.cse.dmu.ac.uk/~mward/
%
% This program is free software; you can redistribute it and/or modify
% it under the terms of the GNU General Public License as published by
% the Free Software Foundation; either version 3 of the License, or
% (at your option) any later version.
%
% This program is distributed in the hope that it will be useful,
% but WITHOUT ANY WARRANTY; without even the implied warranty of
% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
% GNU General Public License for more details.
%
% You should have received a copy of the GNU General Public License
% along with this program; if not, see <http://www.gnu.org/licenses/>.
%
%
% This is the "program" style option which sets up the
% program and programbox environments,
% keywords for programs and a few goodies.
% NOTE: Within the program environment:
% (1) Newlines are significant.
% (2) Each line is in math mode, so for example spaces in the input
%     file are not significant.
% (3) \\ within a line causes a linebreak in the output.
%
% We also define a "programbox" environment which typesets a program in a box.
% Useful for keeping a pice of code on one page or for typesetting small 
% programs in running text.
% We also redefine \( and \) as \begin{programbox} and \end{programbox}.
% The \tab and \untab commands are defined to have no effect while outside 
% a program environment, hence a single-line program can be typeset in 
% maths mode without the overhead associated with programbox.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Section (1). The Keywords.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Set up ";" to add a thick maths space after it when active in math mode:
\let\@semicolon=;
\catcode`\;=12\relax
\mathcode`\;="8000 % Makes ; active in math mode
{\catcode`\;=\active \gdef;{\ifmmode\semicolon\;\else\@semicolon\fi}}
\mathchardef\semicolon="603B

% Set up ` so that ``...'' typesets the string in tt (in math mode):
\mathcode`\`="8000 % Makes ` active in math mode only.
{%\catcode`\'=\active 
 \catcode`\`=\active
 \gdef`{\startstring@}
}
\newif\ifMathsModeStrings \MathsModeStringsfalse
\def\startstring@`#1''{\ifMathsModeStrings
			 \mbox{``}#1\mbox{''}\else
			 \mbox{``{\tt #1}''}\fi}

% Set up a larger array of tabs since programs set lots of tabs.
% This section can be extended if more tabs are needed:
\newdimen\@gtempa 
\chardef\@firsttab=\the\allocationnumber
\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa
\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa
\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa
\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa
\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa
\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa
\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa
\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa
\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa
\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa
\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa
\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa\newdimen\@gtempa
\newdimen\@gtempa 
\chardef\@maxtab=\the\allocationnumber
% NB: can't use \pushtabns and \poptabs to reduce the need for tabs
% since \@curtab, \@curtabmar and \@nxttabmar are global variables
% which would also need to be saved and restored.

% The program environment.
% This is based on the tabbing environment with each line put in math mode,
% \obeylines in force and ";" as an active character.
\def\@programcr{$\@stopline\@startline\ignorespaces$}
\def\programnewpage{$\@stopline\newpage\@startline\ignorespaces$}

% Line numbers on programs:
\newcounter{programline}
\newif\ifNumberPrograms
% Default is no line numbers:
\NumberProgramsfalse

% Program text size hook:
\let\programsize=\relax

% Set switch to false if you want | to act normally 
% outside the program environment:
\newif\ifVBarOutsideProgram \VBarOutsideProgramtrue
\def\normalbaroutside{\catcode`\|=12 \VBarOutsideProgramfalse}

\def\program{%
  \ifNumberPrograms\setcounter{programline}{0}\let\@savecurrentlabel\@currentlabel\fi
  \ifVBarOutsideProgram\else\catcode`\|=\active\fi %% added line
  \if@minipage\else\leavevmode\fi
  \normalshape
  \obeycr %% added line
  % activate tabbing commands:
  \@tabcommandson %% added line
  \global\let\DO=\@oldDO %% added line
  \lineskip \z@\let\>\@rtab\let\<\@ltab\let\=\@settab
  \let\+\@tabplus\let\-\@tabminus\let\`\@tabrj\let\'\@tablab
  \let\\=\@programcr %% changed from \let\\=\tabcr
  \global\@hightab\@firsttab
  \global\@nxttabmar\@firsttab
  \dimen\@firsttab\@totalleftmargin
  \global\@tabpush0 \global\@rjfieldfalse
  \trivlist \item[]%\if@minipage\else\vskip\parskip\fi
  \programsize
  \setbox\@tabfbox\hbox{\rlap{\indent\hskip\@totalleftmargin
    \the\everypar}}\def\@itemfudge{\box\@tabfbox}\@startline\ignorespaces
  $\@gobblecr %% added line
}

\def\endprogram{$\@stopline\ifnum\@tabpush > 0 \@badpoptabs \fi\endtrivlist%
  \restorecr \@tabcommandsoff %% added line
  \ifVBarOutsideProgram\else\catcode`\|=12\fi %% added line
  \ifNumberPrograms\global\let\@currentlabel\@savecurrentlabel\fi
\@gobblecr
}

\def\smallprogram{%
  \let\programsize=\small\program
}

\def\endsmallprogram{%
  \let\programsize=\relax\endprogram
}

% - version which puts the whole program in a box.
\newif\if@programbox \@programboxfalse
\newenvironment{programbox}%
    {\begin{minipage}[t]{\textwidth}%
     \@programboxtrue
     \begin{program}}%
    {\end{program}%
     \@programboxfalse
     \end{minipage}%
}

\def\({\begin{programbox}}
\def\){\end{programbox}}

% A new version of @stopline which ignores blank lines (lines with 
% width 0pt). To print a blank line, put "\ " on it!
%
\def\@stopline{%
  \unskip\@stopfield
  \if@rjfield
    \global\@rjfieldfalse
    \@tempdima\@totalleftmargin \advance\@tempdima\linewidth
    \hbox to\@tempdima{\@itemfudge\@printlineno\hskip\dimen\@curtabmar
		       \box\@curline\hfil\box\@curfield}%
  \else
    \@addfield
    \ifdim\wd\@curline=0pt\else
      \hbox{\@itemfudge\@printlineno\hskip\dimen\@curtabmar\box\@curline}%
  \fi
\fi
}

\def\@printlineno{\ifNumberPrograms
		     \global\def\@currentlabel{\theprogramline}%
		     \hskip\leftmargini
		     \llap{{\prognumstyle(\theprogramline)}\hskip\labelsep}\fi}

\def\prognumstyle{\scriptsize\em}

\def\@startline{\global\@curtabmar\@nxttabmar
   \ifNumberPrograms\grefstepcounter{programline}\fi      % Added by M.Ward
   \global\@curtab\@curtabmar\global\setbox\@curline\hbox % missing \global
    {}\@startfield\strut}                                 % added 17 Jun 86

\def\grefstepcounter#1{\stepcounter{#1}\let\@tempa\protect
  \def\protect{\noexpand\protect\noexpand}%
  \global\edef\@currentlabel{\csname p@#1\endcsname\csname the#1\endcsname}%
  \let\protect\@tempa}
 


% A switch to allow \BAR...\BAR without untabbing twice:
\newif\ifBarDone \BarDonefalse

% a switch to allow \IF or \ELSIF with no \THEN (Grrr...):
\newif\ifTHEN

% For saving and restoring tab numbers (if a structure may contain
% "unbalanced" \tab ... \untab pairs:
\newcount\old@nxttabmar

% These are the commands used to set the tabs.
% They have different definitione inside and outside tebbing environments:

\def\@tabcommandson{% activate tabbing commands:
  % \tab sets a tab stop and adds one to the margin tab:
  \def\tab{$\=\+$}%
  % \qtab sets a tab stop at one quad of indentation:
  \def\qtab{\quad$\=\+$\kern-1em}%
  % \untab removes one tab stop and moves left if at the beginning of a line:
  \def\untab{$\@finishfield\@ifatmargin\@ltab\else\relax\fi\-$}%
  % Must finish current field before testing if at margin:
  \def\@finishfield{\@stopfield\@addfield\@startfield}%
  % \@marginspace adds an extra space unless there is no text on the line:
  \def\@marginspace{$\@finishfield$\@ifatmargin\relax\else\ \fi}%
  % \rcomment{...} provides a comment flush to the right margin:
  \def\rcomment##1{$\`##1$}%
  % \llapm{...} is like \llap{...} but also leaves and re-enters math
  % mode so that "\llapm{stuff}(" does not put any space between the stuff
  % and the "(". This means it will line up with "\llapm{stuff}X"
  % Note this is only used when \@tabcommandson is in force so we are in
  % normal math mode, not display math mode.
  % The 1sp space is so that a line with just an \llapm item on it is not 
  % considered to be empty!
  \def\llapm##1{\@ifatmargin
		  \llap{$##1$}$\hskip 1sp$%
		\else ##1 \fi}%
  \def\savetab{\global\old@nxttabmar\@nxttabmar}
  \def\restoretab{\global\@nxttabmar\old@nxttabmar}
  % Use this to typeset "..." at a higher tab position:
  \def\utdots{$\@finishfield\@ifatmargin\@ltab\@ltab\else\relax\fi$\dots}
  % For typesetting a relation:
  \def\llapr##1{\@ifatmargin
		  \llap{$\ ##1\ $}${}$%
		\else\ ##1\ \fi}%
}

\def\@tabcommandsoff{% deactivate tabbing commands:
  \let\tab=\relax%
  \let\qtab=\relax%
  \let\@finishfield=\relax%
  \let\untab=\relax%
  \let\@marginspace=\ % never at margin thus always a space
  \def\rcomment##1{\qquad\mbox{##1}}%
  \let\savetab=\relax%
  \let\restoretab=\relax%
  \let\utdots=\dots%
  \def\llapm##1{##1}%
  \def\llapr##1{##1}%
}


%% Now for the keywords:

\def\IF{\keyword{if}\global\THENfalse\ \tab}
\def\THEN{\@marginspace\keyword{then}\global\THENtrue\ \tab}
% else has the same width as then and lines up with it on right:
\def\ELSE{\@marginspace\llapm{\keyword{else}\ }}%
% elsf lines up with the if:
\def\ELSF{\@marginspace\untab\ifTHEN\untab\fi%
	  \global\THENfalse\keyword{elsf}\ \tab}
\def\ELSIF{\@marginspace\untab\ifTHEN\untab\fi%
	   \global\THENfalse\keyword{elsif}\ \tab}
% \AR is the arrow for Dijkstra if and do:
% \AR* starts a newline with one quad indentation:
\def\AR{\@marginspace\rightarrow\global\THENtrue\@ifstar%
	{\\\quad\tab\global\BarDonefalse\@gobblecr}%
	{\ \tab\global\BarDonefalse}}%
% bar lines up on right with if or do keyword:
\def\BAR{\@marginspace\ifBarDone\else\untab\fi\global\BarDonetrue
	 \llapm{\barsymbol\ }}%
\def\FI{\@marginspace\untab\ifTHEN\untab\fi\keyword{fi}}
\def\AWAIT{\keyword{await}\ }% \THEN provides the \tab
\def\DO{\keyword{do}\ \tab}
\let\@oldDO=\DO
\def\OD{\@marginspace\untab\keyword{od}}
% \WHILE, \FOR, \FOREACH and \ATEACH temporarily change \DO to not set a tab:
\def\WHILE{\keyword{while}\ \tab
	   \gdef\DO{\@marginspace\keyword{do}\ \global\let\DO=\@oldDO}}
\def\FOR{\keyword{for}\ \tab
	 \gdef\DO{\@marginspace\keyword{do}\ \global\let\DO=\@oldDO}}
\def\FOREACH{\qtab\keyword{foreach}%
	     \gdef\DO{\keyword{do}\ \global\let\DO=\@oldDO}%
	     \ \@typename}
\def\ATEACH{\qtab\keyword{ateach}%
	    \gdef\DO{\keyword{do}\ \global\let\DO=\@oldDO}%
	    \ \@typename}
\def\STEP{\@marginspace\keyword{step}\ }
\def\TO{\@marginspace\keyword{to}\ }
% \BEGIN, \REP, \ACTIONEQ and \WHERE
% make sure next statement starts on a new line
% with one quad of indentation:
\def\BEGIN{\qtab\hbox{\keyword{begin}}\ }%
\def\REP{\qtab\hbox{\keyword{rep}}\ }%
\def\ACTIONEQ{\ \equiv\\\quad\tab}%
\def\WHERE{\@marginspace\untab\qtab\hbox{\keyword{where}}\ }%
\def\IFMATCH{\qtab\keyword{ifmatch}\ \@typename}
\def\FILL{\keyword{fill}\ \tab\savetab\@typename}
\def\ENDFILL{\@marginspace\restoretab\untab\keyword{endfill}}
\def\EDIT{\keyword{edit}\ \tab}
\def\EDITPARENT{\qtab\keyword{editparent}\ }
\def\ENDEDIT{\@marginspace\untab\keyword{endedit}}
\def\ENDMATCH{\@marginspace\untab\untab\keyword{endmatch}}
\def\EXIT{\keyword{exit}}
% Generalised expression brackets:
\def\EXP{\openexp\tab}
\def\ENDEXP{\untab\closexp}
\def\VAR{\qtab\keyword{var}\ }
\def\var{\ \keyword{var}\ }
\def\END{\@marginspace\untab\keyword{end}}
\def\ENDVAR{\@marginspace\untab\keyword{end}}
\def\ENDREP{\@marginspace\untab\keyword{endrep}}
\def\WHERE{\@marginspace\untab\tab\keyword{where}\ }
\def\WITHIN{\@marginspace\untab\keyword{within}\ }
\def\PROC{\qtab\keyword{proc}\ 
	  \gdef\EQ{\EQsymbol\global\let\EQ=\@oldEQ}}
\def\ENDPROC{\fullstop}
\def\FUNCT{\qtab\keyword{funct}\ 
	   \gdef\EQ{\EQsymbol\global\let\EQ=\@oldEQ}}
\def\ENDFUNCT{\fullstop\global\let\EQ=\@oldEQ}
\def\JOIN{\keyword{join}\ \tab}
\def\NIOJ{\@marginspace\untab\keyword{nioj}}
\let\ENDJOIN=\NIOJ
\def\ONEOF{\keyword{oneof}\ \tab}
\def\FOENO{\@marginspace\untab\keyword{foeno}}

\def\ACTIONS{\tab\keyword{actions}\ \global\let\EQ=\@oldEQ}
\def\ENDACTIONS{\@marginspace\untab\keyword{endactions}}
\def\ENDACTION{\fullstop}
\def\CALL{\keyword{call}\ }
\def\LLAC{}
\let\ENDCALL=\LLAC
\def\COMMENT#1{\keyword{comment}\mbox{: #1}}
\def\C#1{\keyword{C}:\ \mbox{#1}}
\def\ARRAY{\keyword{array}\ }
\def\LIKE{\@marginspace\keyword{array}\ }
\def\TYPEDEF{\@marginspace\keyword{typedef}\ }

\def\@typename#1{\mbox{#1}\ }

% The symbols used in programs:
\def\BODY{\EQsymbol}
\def\QE{\fullstop} % end of == definition.

% Expression brackets:
\def\openexp{\mathopen {\mbox{\rule[-0.5ex]{0.04em}{2.3ex}%
			      \rule[1.7ex]{0.4em}{0.1ex}}}}
\def\closexp{\mathclose{\mbox{\rule[-0.5ex]{0.4em}{0.1ex}%
			      \rule[-0.5ex]{0.04em}{2.3ex}}}}

% \fullstop ends an action, proc or funct definition:
\def\fullstop{\untab{\mbox{\bf .}}}
\def\barsymbol{{\rlap{$\sqcap$}\sqcup}}

% \join and \choice symbols:
\def\join{\@marginspace\llapm{\sqcup\ }}%
\def\choice{\@marginspace\llapm{\sqcap\ }}%
% \EQ puts more space around symbol in program environment:
% (this gets redefined by \PROC and \FUNCT):
\def\EQ{\EQsymbol\tab}%
\def\@oldEQ{\EQsymbol\tab}%
\def\EQsymbol{\mathrel{\EQspace\equiv\EQspace}}

% default is tab commands deactivated:
\@tabcommandsoff

% define \normalshape if not present:
\@ifundefined{normalshape}
  {\def\normalshape{\rm}}
  {\relax}

% Underline through descenders:
\let\undertext=\underbar
\def\lowundertext#1{\ifmmode\underline{\vphantom{y}\mbox{#1}}\else
			    $\underline{\vphantom{y}\mbox{#1}}$\fi}

% The Boolean values:
\def\true{\boldvar{true}}
\def\false{\boldvar{false}}

% The simple programs:
\def\ABORT{\boldvar{abort}}
\def\SKIP{\boldvar{skip}}
\def\NULL{\boldvar{null}}

% An abbreviation:
\def\aeq{\ACTIONEQ}

%% Draw a box round something in a program:
\def\progbox#1{%
  % Set #1 in a box, with no tab settings, and restore horizontal position:
  \rlap{\kern-\fboxsep\kern-0.4pt%
	\fbox{$\@tabcommandsoff\phantom{#1}$}}%
  % Then set it again as normal:
  #1\ }

%% For a larger box, covering several lines, put \tl at the top left
%% corner, and \br at the bottom right. THIS REQUIRES pstricks AND pst-node
\def\tl{\llap{\rnode{tl}{\strut}\hspace{2pt}}}
\def\br{\rlap{\hspace{2pt}\rnode{br}{\strut}}%
	      \ncangles[linewidth=0.4pt, linearc=0pt, nodesep=0pt, angle=90,%
			armA=1.5ex, armB=1.5ex]{-}{tl}{br}%
	      \ncangles[linewidth=0.4pt, linearc=0pt, nodesep=0pt, angle=-90,%
			armA=1.4ex, armB=1.4ex]{-}{br}{tl}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Section (2). |Variable_Names|
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% We use an idea from Rainer Schopf's verbatim style
%%% This allows !@#$%^&*() in variable names as well as _
%%% This version should cope better with missing | delimiters:

% First we define the default \variablefont, \variablefontend and \keyword:

\newif\if@corr
\def\no@corr{\do{.}\do{,}}
\def\@corr{\def\do##1{\ifx\temp##1\@corrfalse\fi}\@corrtrue\no@corr
	    \if@corr\/\else\fi\endgroup\egroup} % put back the \egroup

% The old default keyword style is bold underlined:
% The old default variable font is slanted, so \variablefontend adds italic correction:
\def\bfvariables{%
  \let\variablefont=\sl%
  \def\variablefontend##1{\begingroup\futurelet\temp\@corr}% gobble the \egroup
  \def\keyword##1{\mbox{\underbar{\normalshape\bf ##1}}}
  \def\boldvar##1{{\mbox{\normalshape\bf ##1}}}
}

% For sans-serif variables and keywords (no underbar):
\def\sfvariables{%
  \def\variablefont{\normalshape\sf}%
  \def\variablefontend{}%
  \def\keyword##1{\mbox{\normalshape\bf\sf ##1}}%
  \def\boldvar##1{\mbox{\normalshape\bf\sf ##1}}%
}

% For sans-serif variables and keywords in CAPITALS
% (As required for Oberon and Modula)
% This command was submitted by Matteo Corti <corti@inf.ethz.ch>:
\def\bigcaps{%
  \def\variablefont{\normalshape\sf}%
  \def\variablefontend{}%
  \def\keyword##1{\mbox{\uppercase{##1}}}%
  \def\boldvar##1{\mbox{\normalshape\bf\sf ##1}}%
}


% The new default is \sfvariables:

\sfvariables


% Use \scriptvar|foo| for sub/super-script variables:
\def\scriptvariablefont{\scriptsize\@variablefont}%
\def\scriptvar{\let\@variablefont=\variablefont%
	       \let\variablefont=\scriptvariablefont%
	       \let\@variablefontend=\variablefontend%
	       \def\variablefontend{\let\variablefont=\@variablefont%
				    \let\variablefontend=\@variablefontend%
				    \@variablefontend}}

% This section is modified from verbatim.sty:
\newif\ifwasinmmode \wasinmmodefalse
\begingroup
  \lccode`\~=`\^^M
  \lccode`\V=`\V
  \lowercase{%
    \gdef\variable{% first save mmode status:
      \ifmmode\wasinmmodetrue\else\wasinmmodefalse\fi
      \mbox\bgroup\begingroup
      \variablefont
      \catcode`\^^M\active
      \safeat
      \def~{\endgroup\egroup\\
	    \@latexerr{Variable name ended by end of line.}\@ehc}%
      \catcode`\_\active
      \let\do\@makeother
      \do\{\do\}\do\$\do\&%
      \do\#\do\^\do\^^K\do\^^A\do\%\do\~\do\@\@svariable}}
\endgroup
\def\@svariable{%
  \catcode`\|\active
  \lccode`\~`\|%
  \lowercase{\def~{\endgroup% if we were not in mmode, do italic corr:
		   \ifwasinmmode\let\next=\/% was \relax
		     \else\let\next=\variablefontend\fi
		   \next
		   \egroup}%
	     \let\@dovar~}%
  \leavevmode\null}

\catcode`\|=12\relax
\let\origbar=|
\catcode`\|\active

% Make @ active and equal to \char 64:
\begingroup
  \catcode`\@=\active
  \gdef\safeat{\catcode`\@=\active\def@{\char64\relax}}%
\endgroup

\def|{\ifx\@sharp\relax\origbar\else\relax\p@dovar\fi}
\def\p@dovar#1{#1\protect\@dovar\null}
\def\@dovar{\variable} % #1 = \fi from defn of |

%% Set up _ as \_ outside math mode and \sb in math mode:
%% (in case you use _ outside math mode)
\catcode`\_=\active \def_{\ifmmode\sb\else\p@sb\fi}
\def\p@sb{\protect\@sb}
\def\@sb{\_}
% Restore catcode of _ (due to clash with \includegraphics):
\catcode`\_=8


%% Make sure | still works in \verb and verbatim (it is now a "special"):
\def\dospecials{\do\ \do\\\do\{\do\}\do\$\do\&%
  \do\#\do\^\do\_\do\%\do\~\do\|\do\@}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Section (3). Program Schemas.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Definitions for bold subscripted symbols, eg:
%  \B1  or \B{}  or  \B{12} ... etc.
% We check for ' so \B', \S''' etc will work as expected.
\def\A{\boldsub{A}}
\def\B{\boldsub{B}}
\def\P{\boldsub{P}}
\def\Q{\boldsub{Q}}
\def\R{\boldsub{R}}
\def\S{\boldsub{S}}
\def\T{\boldsub{T}}
\def\Z{\boldsub{Z}}

% some bold letters:
\def\d{\boldsub{d}}
\def\e{\boldsub{e}}
\def\t{\boldsub{t}}
\def\w{\boldsub{w}}
\def\x{\boldsub{x}}
\def\y{\boldsub{y}}
\def\z{\boldsub{z}}

\newif\ifMmode \Mmodefalse

\def\boldsub#1{%
  \relax% to fool array and other alignments
  \ifmmode
    \Mmodetrue
  \else
    $\Mmodefalse
  \fi
 \mbox{\normalshape\bf #1}%
 \@boldsub
}

\def\boldsubm#1{%
  \relax% to fool array and other alignments
  \ifmmode
    \Mmodetrue
  \else
    $\Mmodefalse
  \fi
 \boldsymbol{#1}%
 \@boldsub
}

   % Use \mathchoice (typesets all 4) if this is needed for
   % subscripts or superscripts (costs ~0.5 seconds per symbol!):
   % NB use of \text should fix this with AMSLaTeX.
   %\mathchoice{\mbox{\series{bx}\shape{n}\selectfont #1}}%
   %           {\mbox{\series{bx}\shape{n}\selectfont #1}}%
   %           {\mbox{\normalshape\bf\scriptsize #1}}%
   %           {\mbox{\normalshape\bf\tiny #1}}%

\def\@nothing{} \def\prog@prime{'}
\def\@boldsub#1{%
   \def\@boldsubthing{#1}% subscript
   \ifx\@boldsubthing\@nothing% empty
      \let\@boldsubnext\@boldsubfinish
   \else
      \ifx\@boldsubthing\prog@prime%
	 \def\@boldsubnext{^\bgroup\prime\@absorbprimes}%
      \else
	 \def\@boldsubnext{_{#1}\@boldsubfinish}\fi
   \fi
   \@boldsubnext
}

\def\@absorbprimes{\futurelet\@boldsubnext\@seeifprime}
\def\@seeifprime{%
   \ifx\@boldsubnext'%
      \def\@boldsubnext{\@getprime}%
   \else
      \def\@boldsubnext{\egroup\@boldsubfinish}%
   \fi
   \@boldsubnext
}
\def\@getprime'{\prime\@absorbprimes}
\def\@boldsubfinish{\ifMmode\else$\fi}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Section (4). Maths notation used in programs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Notation for sets of the form {...|...} :
% Eg: \set{x \in N | x>0}  becomes:
% \left\{\left.\,  x \in N \:\right\origbar\: x>0 \,\right\}
% set brackets and | grow to fit the size if their contents.
% Also: \bigset{...|...} becomes: 
%                        \bigl\{\, ... \mathrel{\bigm\origbar} ... \, \bigr\}
% \bigset is in an aligned environment, so it can include \\
% (AMSLaTeX only)
%
\def\set#1{\@@set#1\@end} % strip of the {} and pass to \@@set
\def\@@set#1|#2\@end{\left\{\left.\, #1 \:\right\origbar\:
		     #2 \,\right\} }
\def\bigset#1{\@bigset#1\@end} % strip of the {} and pass to \@bigset
\@ifundefined{aligned}
{% Not AMSLaTeX:
  \def\@bigset#1|#2\@end{\bigl\{\, #1 {\:\bigm\origbar\:}
			 #2 \,\bigr\} }
}{% With AMSLaTeX:
  \def\@bigset#1|#2\@end{\begin{aligned}[t]\bigl\{\, #1 {\:\bigm\origbar\:}&
			 \let\@oldcr=\\\def\\{\@oldcr&{}}
			 #2 \,\bigr\} \end{aligned} }
}

% Notation for substitution in programs:
\def\sub[#1/#2|#3]{\left[\left.#1\,/\,#2\,\right\origbar\,#3\,\right]}
\def\bigsub[#1/#2|#3]{\bigl[#1\,\bigm/\,#2\,\bigm\origbar\,#3\,\bigr]}
% Use \modbar{x} for |x|:
\def\modbar#1{\left\origbar #1\right\origbar}

% Notation for a sequence in angle brackets:
% \bigseq uses big size of brackets:
% \def\seq#1{\left< #1 \right>}
\def\seq#1{\langle #1 \rangle}
\def\bigseq#1{\bigl< #1 \bigr>}

% Notation for subsequences analogous to set notation:
\def\subseq#1{\@@subseq#1\@end} % strip of the {} and pass to \@@subseq
\def\@@subseq#1|#2\@end{\left<\left.\, #1 \:\right\origbar\:
			#2 \,\right>}
\def\bigsubseq#1{\@bigsubseq#1\@end} % strip of the {} and pass to \@bigsubseq
\@ifundefined{aligned}
{% Not AMSLaTeX:
  \def\@bigsubseq#1|#2\@end{\bigl<\, #1 {\:\bigm\origbar\:}
			    #2 \,\bigr> }
}{% With AMSLaTeX:
  \def\@bigsubseq#1|#2\@end{\begin{aligned}[t]\bigl<\, #1 {\:\bigm\origbar\:}&
			    \let\@oldcr=\\\def\\{\@oldcr&{}}
			    #2 \,\bigr> \end{aligned} }
}

% range dots, like \ldots but with two dots only (for 1..n etc.):
\def\rdots{\mathinner{\ldotp\ldotp}}

% Atomic Specification statement: for eg <x>/<y>.Q use: \atspec x/y. Q
% This uses "/" and "." as argument delimiters:
% \def\atspec #1/#2.{\seq{#1}\!/\!\seq{#2}\!.}
\def\atspec #1/#2.{\seq{#1}/\seq{#2}.}

% \Forall vars.formula and \Exists vars.formula:
\def\Forall#1.{\forall #1.\,}
\def\Exists#1.{\exists #1.\,}

\let\EQspace=\  % default space around \EQ \EQT and \LE
\def\EQT{\mathrel{\EQspace\approx\EQspace}}      % program equivalence.
\def\LE{\mathrel{\EQspace\le\EQspace}}           % program refinement.
\def\SLE{\mathrel{\EQspace\preccurlyeq\EQspace}} % semi-refinement.
\def\NOT{\neg}
% \AND and \OR relations have an extra thin space around them:
\def\AND{\mathrel{\,\wedge\,}}
\def\OR{\mathrel{\,\vee\,}}
\def\EOR{\mathrel{\,\oplus\,}}
\def\sbs{\subseteq}
\def\im{\Rightarrow}
% (use \iff and \implies for the "long" arrows)
\def\union{\cup}
\def\intersect{\cap}
\def\lar{\leftarrow}
\def\rar{\rightarrow}
\def\wflt{\prec}
\def\wfle{\preccurlyeq}
\def\succstar{\mathrel{\succ\!\!^*}}
\def\succeqstar{\mathrel{\succeq\!^*}}
\def\gt{\ifmmode>\else{$>$}\fi}
\def\lt{\ifmmode<\else{$<$}\fi}
\def\tw{\ifmmode{}^\sim\else{${}^\sim$}\fi}


% map and reduce operators:
\def\bstar{\mathrel{\boldsymbol{*}}} % for *
\def\bdiv{\boldsymbol{/}} % for /


% Various arrows (taken from oz.sty):
\let \rel       \leftrightarrow
\let \tfun      \rightarrow
\let \tinj      \rightarrowtail
\def \tsur      {\mathrel{\ooalign{$\tfun$\hfil\cr$\mkern4mu\tfun$}}}
\def \pfun      {\p\tfun}
\def \pinj      {\p\tinj}
\def \psur      {\p\tsur}
\def \ffun      {\f\tfun}
\def \finj      {\f\tinj}
\def \bij       {\mathrel{\ooalign{$\tinj$\hfil\cr$\mkern5mu\tfun$}}}
\def\p#1{\mathrel{\ooalign{\hfil$\mapstochar\mkern 5mu$\hfil\cr$#1$}}}
\def\f#1{\mathrel{\ooalign{\hfil
	$\mapstochar\mkern 3mu\mapstochar\mkern 5mu$\hfil\cr$#1$}}}

%% Logical exclusive or:
\def\exor{\oplus}

%% Sequence concatenation:
\def\concat{\mathrel{+\!\!\!+}}

\def\rmtiny{\normalshape\rm\tiny}

%% Stack operations:
\def\push{\mathrel{\overset{\mbox{\rmtiny push}}{\longleftarrow}}}
\def\pop {\mathrel{\overset{\mbox{\rmtiny  pop}}{\longleftarrow}}}
\def\pick{\mathrel{\overset{\mbox{\rmtiny pick}}{\longleftarrow}}}
\def\last{\mathrel{\overset{\mbox{\rmtiny last}}{\longleftarrow}}}

%% bitwise operators
\def\bitand {\mathrel{\overset{\mbox{\tiny bit}}{\wedge}}}
\def\bitor  {\mathrel{\overset{\mbox{\tiny bit}}{\vee}}} 
\def\bitexor{\mathrel{\overset{\mbox{\tiny bit}}{\vphantom\vee\smash\oplus}}}
\def\bitnot{{\overset{\mbox{\tiny bit}}{\vphantom\vee\neg}}}

%% Logical, decimal and floating point operators:
\def\lplus {\mathrel{\overset{\mbox{\tiny log}}{+}}}
\def\lminus{\mathrel{\overset{\mbox{\tiny log}}{-}}}
\def\lmult {\mathrel{\overset{\mbox{\tiny log}}{\times}}}
\def\ldiv  {\mathrel{\overset{\mbox{\tiny log}}{\div}}}
\def\lequ  {\mathrel{\overset{\mbox{\tiny log}}{=}}}
\def\lneq  {\mathrel{\overset{\mbox{\tiny log}}{\neq}}}
\def\lless {\mathrel{\overset{\mbox{\tiny log}}{<}}}
\def\lgreat{\mathrel{\overset{\mbox{\tiny log}}{>}}}
\def\lleq  {\mathrel{\overset{\mbox{\tiny log}}{\leq}}}
\def\lgreq {\mathrel{\overset{\mbox{\tiny log}}{\geq}}}
\def\dplus {\mathrel{\overset{\mbox{\tiny dec}}{+}}}
\def\dminus{\mathrel{\overset{\mbox{\tiny dec}}{-}}}
\def\dmult {\mathrel{\overset{\mbox{\tiny dec}}{\times}}}
\def\ddiv  {\mathrel{\overset{\mbox{\tiny dec}}{\div}}}
\def\deq   {\mathrel{\overset{\mbox{\tiny dec}}{=}}}
\def\dneq  {\mathrel{\overset{\mbox{\tiny dec}}{\neq}}}
\def\dless {\mathrel{\overset{\mbox{\tiny dec}}{<}}}
\def\dgreat{\mathrel{\overset{\mbox{\tiny dec}}{>}}}
\def\dleq  {\mathrel{\overset{\mbox{\tiny dec}}{\leq}}}
\def\dgreq {\mathrel{\overset{\mbox{\tiny dec}}{\geq}}}
\def\fplus {\mathrel{\overset{\mbox{\tiny fpt}}{+}}}
\def\fminus{\mathrel{\overset{\mbox{\tiny fpt}}{-}}}
\def\fmult {\mathrel{\overset{\mbox{\tiny fpt}}{\times}}}
\def\fdiv  {\mathrel{\overset{\mbox{\tiny fpt}}{\div}}}
\def\feq   {\mathrel{\overset{\mbox{\tiny fpt}}{=}}}
\def\fneq  {\mathrel{\overset{\mbox{\tiny fpt}}{\neq}}}
\def\fless {\mathrel{\overset{\mbox{\tiny fpt}}{<}}}
\def\fgreat{\mathrel{\overset{\mbox{\tiny fpt}}{>}}}
\def\fleq  {\mathrel{\overset{\mbox{\tiny fpt}}{\leq}}}
\def\fgreq {\mathrel{\overset{\mbox{\tiny fpt}}{\geq}}}

%% mod and div:
\def\MOD{\mathrel{\text{mod}}}
\def\DIV{\mathrel{\text{div}}}

%% add the definition of overset if not present:
\@ifundefined{overset}%
  {\def\overset#1#2{\binrel@{#2}%
     \binrel@@{\mathop{\kern\z@#2}\limits^{#1}}}
   \def\binrel@#1{\setboxz@h{\thinmuskip0mu
      \medmuskip\m@ne mu\thickmuskip\@ne mu$#1\m@th$}%
     \setbox@ne\hbox{\thinmuskip0mu\medmuskip\m@ne mu\thickmuskip
      \@ne mu${}#1{}\m@th$}%
     \setbox\tw@\hbox{\hskip\wd@ne\hskip-\wdz@}}
   \def\binrel@@#1{\ifdim\wd2<\z@\mathbin{#1}\else\ifdim\wd\tw@>\z@
     \mathrel{#1}\else{#1}\fi\fi}%
   \def\setboxz@h{\setbox\z@\hbox}%
   \def\setbox@ne{\setbox\@ne}%
   \def\wd@ne{\wd\@ne}%
   \def\wdz@{\wd\z@}%
  }{}

%% =df symbol (with thick space around it):
\def\edf{\mathrel{\;=_{{}_{\mbox{\rmtiny DF}}}\;}}

%% empty set symbol: (use \varnothing if available)
\@ifundefined{varnothing}%
	     {\let\nullset=\emptyset}%
	     {\let\nullset=\varnothing}%

%% Powerset symbol:
\@ifundefined{DeclareMathSymbol}{%
%% check if \teurm defined - if not then use \oldwp (Large and raised):
\@ifundefined{teurm}%
  {\def\powerset{\raisebox{0.5ex}{\Large$\oldwp$}}}% no \eurm
  {\def\powerset{\raisebox{0.5ex}{\Large\teurm\char"7D}}}% Use Euler roman p
}{%
\DeclareSymbolFont{eulerletters}{U}{eur}{m}{n}%
\DeclareMathSymbol{\powersetsymbol}{\mathord}{eulerletters}{"7D}%
\newsavebox{\powersetbox}
\sbox{\powersetbox}{\raisebox{0.5ex}{\mbox{\Large$\powersetsymbol$}}}
\def\powerset{\usebox{\powersetbox}}
% old defn -- with amslatex this makes the whole maths item \Large!
%\def\powerset{\raisebox{0.5ex}{\Large$\powersetsymbol$}}
}%


%% The stmaryrd style and fonts include \bigsqcap, but if you don't have
%% it, here is an alternative using rules (only works at standard size):
\@ifundefined{bigsqcap}
  {\def\bigsqcap{\mathop{%
		\rule[-0.2ex]{.07em}{2.17ex}%
		\rule[1.8ex]{0.5em}{.17ex}%
		\rule[-0.2ex]{.07em}{2.17ex}}}}
  {\relax}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Section (5). Miscellaneous bits and pieces
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%% Substitute for some AMSLaTeX things if they are missing:
\@ifundefined{text}{\let\text=\mbox}{}
\@ifundefined{boldsymbol}{\def\boldsymbol#1{\mbox{\bf #1}}}{}
\@ifundefined{implies}{\def\implies{\;\Longrightarrow\;}}{}
\@ifundefined{operatorname}{\def\operatorname#1{\mathop{#1}}}{}


% \snugbox is by Victor Eijhout, eijkhout@cs.utk.edu, TUGboat 13, 1, 1992.
% It sets a box containing paragraphs as wide ``as it really is''
\def\snugbox{\mbox\bgroup
%            ^^^^^ changed from \hbox by M.Ward
  \setbox\z@\vbox\bgroup
    \leftskip\z@
    \bgroup\aftergroup\make@snug
    \let\next=}
\def\make@snug{\par\sn@gify\egroup
  \box\z@\egroup}
\def\sn@gify
  {\skip\z@=\lastskip \unskip
   \advance\skip\z@\lastskip \unskip
   \unpenalty
   \setbox\z@\lastbox
   \ifvoid\z@ \nointerlineskip
     \else {\sn@gify} \fi
   \hbox{\unhbox\z@}\nointerlineskip
   \vskip\skip\z@
   }
% To vertically centre the box:
\def\textvcenter{\hbox\bgroup$
  \everyvbox{\everyvbox{}%
    \aftergroup$%
    \aftergroup\egroup}
  \vcenter}


%% Cases environment:
%% based on description environment with numbering:
\def\Cases{
  \ifnum \@enumdepth >3 \@toodeep\else
    \advance\@enumdepth \@ne
    \edef\@enumctr{enum\romannumeral\the\@enumdepth}%
     \@ifundefined{mathindent}
     {\list{\kern-1em\hbox{\normalshape\bf Case \arabic{\@enumctr}:}}%
	   {\usecounter{\@enumctr}%
	     \def\makelabel##1{##1}}}%
     {\list{\kern-1em\hbox{\normalshape\bf Case \arabic{\@enumctr}:}}% 
	   {\mathindent 0pt \usecounter{\@enumctr}%
	     \def\makelabel##1{##1}}}%
  \fi}

\let\endCases=\endlist

%% \CASES is redundant with amstex.sty
\def\CASES#1{\left\{\,\vcenter{{\let\\=\cr\normalbaselines\m@th
    \ialign{$##\hfil$&\quad##\hfil\crcr#1\crcr}}}\right.}

%% Environment romanenumerate for lists numbered by roman numerals:
\def\romanenumerate{\begingroup
  \def\theenumi{\normalshape(\myroman{enumi})}%
  \def\p@enumi{}%
  \def\labelenumi{\theenumi}%
  \enumerate}
\def\endromanenumerate{\endenumerate\endgroup}

%% A fix to get lower case Roman numerals for use as labels:
\def\myroman#1{\@myroman{\@nameuse{c@#1}}}
\def\@myroman#1{\expandafter{\romannumeral #1}}

%% \proof macro for theorems and lemmas:
\def\proof{\normalshape{\setlength{\parskip}{0pt}\par\addvspace\medskipamount
			\noindent{\bf Proof: }}\ignorespaces}

%% require the {...} for \wp and \WP
\let\oldwp=\wp % save old \wp (curly p character)
%\def\wp#{\@wp}
%\def\@wp#1{\mbox{\normalshape wp}(#1)}
%\def\WP#{\@WP}
%\def\@WP#1{\mbox{\normalshape WP}(#1)}
%% Don't require {...}, ie use normal parentheses where required:
\def\wp{\mbox{\normalshape wp}}
\def\WP{\mbox{\normalshape WP}}


%% Two line displayed equation, eg:
%% \[  \twoline{ a_very_long_left_hand_side \\
%%                   {} = a_fairly_long_right_hand_side } \]
%% Use in displayed maths mode.
%% NB this is superseded by AMSLaTeX's multline environment.
\def\twoline#1{\def\\{\hfill\cr\hfill}% \def only lasts to end of display
	       \displaylines{\quad #1 \quad\cr}}

%% Add a definition of \Bbb if not present:
% We use poor man's bold to give an ``extra bold'' letter:
\@ifundefined{Bbb}
  {\def\Bbb{\protect\pBbb}
   \def\pBbb#1{\setbox0=\hbox{\bf #1}
	       \kern-.025em\copy0\kern-\wd0
	       \kern.05em\copy0\kern-\wd0
	       \kern-.025em\raise.0433em\box0 }}
  {\relax}

%% Add a definition of cases environment if not present:
\@ifundefined{endcases}
  {\def\cases{\left\{\def\arraystretch{1.2}\hskip-\arraycolsep
     \array{l@{\quad}l}}
   \def\endcases{\endarray\hskip-\arraycolsep\right.}}
  {\relax}

%% draw a line across the page:
\def\dashes{$\makebox[6in]{\hrulefill}$}

%% A \qed command for the end of a proof:
\@ifundefined{blacksquare}
  {\def\qedsymbol{\vrule width.6em height.5em depth.1em\relax}}
  {\let\qedsymbol=\blacksquare}
\def\qed{\ifx\\\@eqncr\let\next\eqnarrayqed\else
  \ifmmode\let\next\eqnqed\else
    \let\next\textqed\fi\fi\next}
%\def\eqnqed#1\]{\belowdisplayskip\z@\belowdisplayshortskip\z@
%  \postdisplaypenalty\@M\relax#1
%  \]\par{\lineskip\z@\baselineskip\z@\vbox to\z@{\vss\noindent\textqed}}} 
%% simpler version from ROGERS@se.physto.vana using the primitive \eqno:
\def\eqnqed#1\]{\relax#1\eqno\qedsymbol$$\ignorespaces}
\def\textqed{{\unskip\nobreak\hfil\penalty50\hskip2em\null\nobreak\hfil
	      $\qedsymbol$\parfillskip\z@\finalhyphendemerits0\par}}
\def\eqnarrayqed{\\\noalign{\vspace{-\jot}%
  {\lineskip\z@\baselineskip\z@%
    \vbox to\z@{\vss\noindent\textqed}}%
  \vspace{-\baselineskip}}}


%% A crude method of allowing URLs to break across lines: sprinkle ~'s
%% inside your \www{...} command, eg:
%% \www{http://~ws-mj3.~dur.~ac.~uk/~martin/~papers/~ref-ws-5.ps.gz}

\def\www{\bgroup\def~{\hskip 1pt plus 3pt minus 1pt\relax}\www@}
\def\www@#1{$\langle$#1$\rangle$\egroup}

%% Fix the use of | in \index:

\def\makeindex{%
  \newwrite\@indexfile
  \immediate\openout\@indexfile=\jobname.idx
  \def\index{\@bsphack\begingroup
	      \catcode`\|=12
             \@sanitize
             \@wrindex}\typeout
    {Writing index file \jobname.idx}%
  \let\makeindex\@empty
}
\def\index{\@bsphack\begingroup\catcode`\|=12\@sanitize\@index}



==> related.tex <==
\begin{figure}[tb!]
\begin{center}
\footnotesize
\begin{tabular}{l @{\hspace{1pt}}|@{\hspace{2pt}} l}
\underline{Variant 4 (Elemental)} & \underline{Variant 4 (ScaLAPACK)} \\
$
  \begin{array}[t]{l}
    A_{10} \becomes L_{11}^{-1} A_{10} \\
\rowcolor[gray]{0.7}    A_{20} \becomes A_{20} - L_{21} A_{10} ~~~ \mbox{(gemm)} \\
\rowcolor[gray]{0.9}    A_{11} \becomes L_{11}^{-1} A_{11} L_{11}^{-H} \\
    Y_{21} \becomes L_{21} A_{11} \\
    A_{21} \becomes A_{21} L_{11}^{-H} \\
    A_{21} \becomes W_{21} = A_{21}  - \frac{1}{2} Y_{21} \\
\rowcolor[gray]{0.7}    A_{22} \becomes A_{22} - ( L_{21} A_{21}^H + A_{21} L_{21}^H ) ~~~ \mbox{(her2k)} \\
%    A21 =  A21 + Y21;
    A_{21} \becomes A_{21} - \frac{1}{2} Y_{21}  \\
  \end{array}
$ 
&
$
  \begin{array}[t]{l}
    G_{21} \becomes L_{21} \\
    R_{21} \becomes A_{21} \\
    S_{10} \becomes A_{10} \\
    R_{11} \becomes \mbox{tril}(A_{11}) \\
    G_{21} \becomes -G_{21} L_{11}^{-1} \\
    R_{21} \becomes R_{21} + \frac{1}{2} G_{21} A_{11} \\
    \rowcolor[gray]{0.7}  A_{22} \becomes A_{22} + G_{21} R_{21}^H + R_{21} G_{21}^H  ~~~ \mbox{(her2k)} \\
    \rowcolor[gray]{0.7}  A_{20} \becomes A_{20} + G_{21} S_{10} ~~~ \mbox{(gemm)} \\
    A_{21} \becomes A_{21} + G_{21} R_{11} \\
    A_{10} \becomes L_{11}^{-1} A_{10} \\
\left. 
\begin{array}{@{}l}
\rowcolor[gray]{0.9}    C_{11} \becomes \mbox{tril}(A_{11}) \\
\rowcolor[gray]{0.9}    \mbox{triu}(C_{11}) := \mbox{tril}(C_{11})^H \\
\rowcolor[gray]{0.9}     C_{11} \becomes L_{11}^{-1} C_{11} \\
\rowcolor[gray]{0.9}     C_{11} \becomes C_{11} L_{11}^{-1} \\
\rowcolor[gray]{0.9}     \mbox{tril}(A_{11}) := \mbox{tril}(C_{11}) 
\end{array} 
\hspace{-0.05in}
\right\} A_{11} \becomes L_{11}^{-1} A_{11} L_{11}^{-H} \\
    A_{21} \becomes A_{21} L_{11}^{-H}
  \end{array}
$ 
\end{tabular}
\vspace{0.1in}
\end{center}
\caption{Operations performance by Variant 4 in Elemental (left) and ScaLAPACK (right).}
\label{fig:ElementalVsSL}
\end{figure}

Variant 4 for $ L^{-1} A L^{-H} $, as implemented in ScaLAPACK routines
{\tt p[sd]syngst} and  {\tt p[cz]hengst},
appears to have been derived from the work by 
by Sears et al.
%%%The algorithm in the paper by Sears et al.\ computes $ L^{-H} A L^{-1} $ 
%%%after having computed a somewhat unusual version of the Cholesky factorization:
%%% $ B = L^H L $.  The paper gives few clues about what motivated the 
%%% discovery of the algorithm.  The algorithm itself is presented as a 
%%% double-nested loop around vector operations so that even level-2 BLAS operations
%%% are not obvious. No blocked algorithm is given in the paper.  It is merely 
%%% mentioned that the unblocked algorithm that is given motivated a blocked 
%%%version.  The one hint at how the algorithm came to be is the mentioning of 
%%% ``Gauss transforms''. We conclude that the authors used the following insight:
%%% When factoring a square matrix $ A $ into its $ LU $ factorization, $ A = L U $,
%%% one can view the process as
%%% \[
%%% \begin{array}[t]{c}
%%% \underbrace{\hat{L}_{n-1} \cdots \hat{L}_0} \\
%%% L^{-1}
%%% \end{array}
%%% A = U ,
%%% \mbox{ where }
%%% \hat{L}_k
%%% = 
%%% \FlaThreeByThreeBR
%%%   { I_{k \times k} }{ 0 }{ 0 }
%%%   { 0 }{ 1 }{ 0 }
%%%   { 0 }{-l_{21}^{(k)}}{ I }
%%% \]
%%% is a Gauss transform.  (Here $ I_{k \times k} $ denotes a $ k \times k $
%%% identity matrix.)
%%% There is a simple relation between $ L $ and these Gauss transforms in that
%%% each $ l_{21}^{(k)} $ equals the corresponding subdiagonal elements of
%%% matrix $ L $.
%%% Thus, the inverse of a {\em unit} lower triangular matrix $ L $ can 
%%% be viewed as a sequence of Gauss transforms that are easily identified from
%%% the matrix $ L $.
%%% If one wishes to compute $ L^{-1} A L^{-H} $ one
%%% can instead compute
%%% $
%%% \left( \hat{L}_{n-1} \cdots \left( \hat{L}_0  A 
%%% \hat{L}_{0}^H \right) \cdots \hat{L}_{n-1}^H \right) $.
%%% %There are a few details beyond this insight, like how to modify this for the
%%% %$ L $ from the Cholesky factorization which is not unit lower triangular and
%%% %how to generalize this to a blocked algorithm.
%%% The paper contains a few details beyond this insight, like how to modify
%%% this algorithm for the $ L $ from the Cholesky factorization, which is not
%%% unit lower triangular, and how to generalize this to a blocked algorithm.
%%% %These are only barely discussed in~\cite{Sears98} nor will we discuss this here, since 
%%% %we have an alternative way for deriving the algorithm.
%%% However, these topics are only barely discussed in~\cite{Sears98}, and we
%%% choose to omit discussion here since we have an alternative way of deriving
%%% the algorithm.
%%% Hopefully, this gives the reader some idea of how the authors
%%% of~\cite{Sears98} may have derived
%%% their algorithm as an alternative to our derivation based on the
%%% FLAME methodology.  
%%% It appears that the routines {\tt p[sd]syngst} and {\tt p[cz]hengst} in ScaLAPACK were 
%%% derived from the work by Sears et al.. 
There are a few subtle differences 
between the algorithm used by those routines and Variant~4 in 
Figure~\ref{fig:algs}, as illustrated in Figure~\ref{fig:ElementalVsSL}.
%%% The two algorithms are essentially the same: 
Expansion of each of the dark 
gray updates in terms of the states of $A$ and $L$ at the beginning of the 
iteration reveals that they are identical. Likewise, the light gray 
update on the right is merely an expanded version of the update 
$A_{11} := L_{11}^{-1} A_{11} L_{11}^{-H}$ that could have been 
performed more simply via a call to LAPACK's {\tt [sd]sygs2} or {\tt [cz]hegs2} routines. 



